Approximation with Error Bounds in Spark

We introduce a sampling framework to support approximate computing with estimated error bounds in Spark. Our framework allows sampling to be performed at the beginning of a sequence of multiple transformations ending in an aggregation operation. The framework constructs a data provenance tree as the computation proceeds, then combines the tree with multi-stage sampling and population estimation theories to compute error bounds for the aggregation. When information about output keys are available early, the framework can also use adaptive stratified reservoir sampling to avoid (or reduce) key losses in the final output and to achieve more consistent error bounds across popular and rare keys. Finally, the framework includes an algorithm to dynamically choose sampling rates to meet user specified constraints on the CDF of error bounds in the outputs. We have implemented a prototype of our framework called ApproxSpark, and used it to implement five approximate applications from different domains. Evaluation results show that ApproxSpark can (a) significantly reduce execution time if users can tolerate small amounts of uncertainties and, in many cases, loss of rare keys, and (b) automatically find sampling rates to meet user specified constraints on error bounds. We also explore and discuss extensively trade-offs between sampling rates, execution time, accuracy and key loss.

==> background.tex <==
\section{Background}
\guangyannote{this entire section can probably be cut}
Spark has emerged as a popular big data processing engine. Essentially, Spark 
extends the map reduce programming model with its main data abstraction called {\em resilient distributed datasets} (RDDs), which are fault-tolerant 
collections of data partitioned across a cluster that can be processed in 
parallel ~\cite{Zaharia2010}. RDDs can also be cached in memory for faster processing. Every Spark application consists of a driver program which converts the application's code containing operations into a 
series of tasks. There are two primary operations which can be performed on RDDs: \textit{transformation} and \textit{actions}. \textit{Transformations} change one RDD into another. The Spark API provides several transformations such as \textit{map}, \textit{filter} and \textit{flatMap}. \textit{Actions} starts computation on an RDD . Some commonly used \textit{actions} are \textit{reduce}, \textit{collect} and \textit{count}. Transformations are lazily evaluated, which means their computations are postponed until an action requires a result to be computed.

The driver program requests resources from a Spark cluster manager, which orchestrates resource allocation across applications in a Spark cluster.
The cluster manager then launches executors, processes that run an instance of
a Java Virtual Machine (JVM), which are used to execute tasks sent by the driver
program. Each executor maintains a cache which stores the most frequently used 
data and therefore avoids costly disk operations. The driver program also schedules
future tasks based on data placement by tracking the location of cached data. 
Another performance improvement is that executors allow new tasks to be started 
quickly since they remain running for the duration of the application.


%\begin{figure}
%	\vspace{0cm}
%	\begin{center}
%		\includegraphics[width=3in]{../approxfigures/Figures/samplingIllustration.pdf} \\
%	\end{center}
%	\vspace{0.25in}
%	\caption{\em A simple Spark transformation, blue boxes are the partitions inside the RDDs}
%	\label{fig:example-spark}
%\end{figure}
%Figure~\ref{fig:example-spark} shows a Spark program that creates an RDD from a dataset, transforms it into a second RDD, then performs a summation to produce a result which is then returned to the driver program or saved to the disk.
{\tiny }
\iffalse

\guangyannote{cut the following paragraphs?}
\myparagraph{Performance} Sometimes only using Spark's \textit{sample} operator is not going to save significant run time for certain jobs, only if the later operations are very expensive. Since {\tt sample} and {\tt sampleByKey} do not drop input blocks, Spark still has to perform expensive I/O on all input blocks when reading the dataset. \textit{runApproximateJob} allows user to explicitly set a time limit for job execution, the unfinished tasks are simply discarded when the time limit hits, which actually wastes computing resources in terms of CPU time and energy.

\myparagraph{Stratified Sampling} Since the user has to specify a sampling rate for each key in the RDD to use {\tt sampleByKey}, if there are many different keys, providing sampling rates for each individual key could be very cumbersome, or even impossible, if the key space is unknown. As mentioned before, it could still entirely miss a key since it relies on Bernoulli Sampling. \textit{sampleByKeyExact} addresses this issue but it has to make an additional pass over all data items, but it also requires the user to specify sampling rates for all keys and it incurs more overhead.

\myparagraph{Confidence interval estimation} As of version $2.1.0$, Spark does not provide the user with confidence intervals if the user samples an RDD by calling {\tt sample} or  {\tt sampleByKey}. In the end, Spark just returns a computed value over the sample. Therefore, the user will not know the estimated value explicitly as well as how much confidence should be placed over the estimated value. 
\fi


==> powerAllocation.tex <==
\section{Optimal allocation for stratified reservoirs}
\label{sec:ASRSOptimal} 
Under the power allocation technique with power $q$ setting to $0$, we compute the reservoir size $|r_{i}|$ for key $i$ as \cite{al2014adaptive}:
\begin{equation}
|r_{i}| = |r| \times\frac{\sigma_{i}/(\frac{\sum_{j=1}^{|R_{i}|}y_{ij}}{|R_{i}|})}{\sum_{k=1}^n\sigma_{k}/(\frac{\sum_{j=1}^{|R_{k}|}y_{kj}}{|R_{k}|})}
\label{eq:resSize}
\end{equation}
where $|R_{i}|$ is the population size of key $i$ and $y_{ij}$ is the $j^{th}$ item value of key $i$ and $\sigma_{i}$ is the standard deviation of key $i$. Then at any point in time $t$ during the sampling process, reservoir size $|r_i(t)|$ is determined by this formula \cite{al2014adaptive}:
\begin{equation}
|r_{i}(t)| = |r| \times\frac{\sigma_{i}(t)/(\frac{\sum_{j=1}^{|S_{i}(t)|}y_{ij}}{|S_{i}(t)|})}{\sum_{k=1}^n\sigma_{k}(t)/(\frac{\sum_{j=1}^{|S_{k}(t)|}y_{kj}}{|S_{k}(t)|})}
\label{eq:resSizeT}
\end{equation}
where $|r_{i}(t)|$ denotes the size of a sub-sample allocated for key $S_{i}$ at time point t, $\sigma_{i}(t)$ denotes the running standard deviation of key $i$ up to t,and $|S_{i}(t)|$ denotes the number of tuples processed up to t from key $i$.
